Mission Level Uncertainty in Multi-Agent Resource Allocation

In recent years, a significant research effort has been devoted to the design of distributed protocols for the control of multi-agent systems, as the scale and limited communication bandwidth characteristic of such systems render centralized control impossible. Given the strict operating conditions, it is unlikely that every agent in a multi-agent system will have local information that is consistent with the true system state. Yet, the majority of works in the literature assume that agents share perfect knowledge of their environment. This paper focuses on understanding the impact that inconsistencies in agents' local information can have on the performance of multi-agent systems. More specifically, we consider the design of multi-agent operations under a game theoretic lens where individual agents are assigned utilities that guide their local decision making. We provide a tractable procedure for designing utilities that optimize the efficiency of the resulting collective behavior (i.e., price of anarchy) for classes of set covering games where the extent of the information inconsistencies is known. In the setting where the extent of the informational inconsistencies is not known, we show -- perhaps surprisingly -- that underestimating the level of uncertainty leads to better price of anarchy than overestimating it.

==> archived/archive.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%% LaTeX Template for AAMAS-2021 (based on sample-sigconf.tex)
% %%% Prepared by Natasha Alechina and Ulle Endriss (version 2020-08-06)

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%% Start your document with the \documentclass command.
% %%% Use the first variant below for the final paper.
% %%% Use the second variant below for submission.

% \documentclass[sigconf]{aamas} 
% %\documentclass[sigconf,anonymous]{aamas} 

% %%% Load required packages here (note that many are included already).

% \usepackage{balance} % for balancing columns on the final page
% \usepackage{amsmath}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%% AAMAS-2021 copyright block (do not change!)

% \setcopyright{ifaamas}
% \acmConference[AAMAS '21]{Proc.\@ of the 20th International Conference on Autonomous Agents and Multiagent Systems (AAMAS 2021)}{May 3--7, 2021}{London, UK}{U.~Endriss, A.~Now\'{e}, F.~Dignum, A.~Lomuscio (eds.)}
% \copyrightyear{2021}
% \acmYear{2021}
% \acmDOI{}
% \acmPrice{}
% \acmISBN{}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%% Use this command to specify your EasyChair submission number.
% %%% In anonymous mode, it will be printed on the first page.

% \acmSubmissionID{637}

% %%% Use this command to specify the title of your paper.

% \title{Multiagent Operations with Informational Inconsistencies }

% %%% Provide names, affiliations, and email addresses for all authors.

% \author{Rohit Konda}
% \affiliation{
%   \institution{University of California, Santa Barbara}
%   \department{Electrical and Computer Engineering}
%   }
% \email{rkonda@ucsb.edu}

% \author{Rahul Chandan}
% \affiliation{
%   \institution{University of California, Santa Barbara}
%   \department{Electrical and Computer Engineering}
%   }
% \email{rchandan@ucsb.edu}

% \author{Jason Marden}
% \affiliation{
%   \institution{University of California, Santa Barbara}
%   \department{Electrical and Computer Engineering}
%   }
% \email{jrmarden@ucsb.edu}

% %%% Use this environment to specify a short abstract for your paper.

% \begin{abstract}
% In this paper we consider a multiagent system operating in a vast environment seeking to accomplish a given system-level objective, e.g., surveillance or perimeter defense.  The operations of such systems require each individual agent to make local decisions in response to locally available information, which could pertain to information regarding the state of the mission or the behavior of the other agents in the system.  Given the vastness and complexity of these systems, it may be the case that the information available to each agent is outdated or inconsistent with the true state of the system. Accordingly, the focus of this paper is on understanding the impact of these informational inconsistencies on the resulting control design and performance guarantees.  More specifically, we consider the design of multiagent operations through a game theoretic lens where the individual agents are assigned localized objective functions to guide their individual behavior.  We provide a tractable procedure for designing these localized objectives that optimizes the efficiency of the resulting collective behavior for situations where the agents can only approximate these localized objectives.  Here, we use Nash equilibria as a model of the emergent collective behavior and the well-studied price of anarchy as a measure of system performance.    
% \end{abstract}

% %%% The code below was generated by the tool at http://dl.acm.org/ccs.cfm.
% %%% Please replace this example with code appropriate for your own paper.


% %%% Use this command to specify a few keywords describing your work.
% %%% Keywords should be separated by commas.

% \keywords{Game Theory, Incomplete Information, Optimization, Resource Allocation}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%% Include any author-defined commands here.

% \newtheorem{thm}{Theorem}%[section]
% \newtheorem{prop}{Proposition}%[section]
% \newtheorem{cor}{Corollary}%[theorem]
% \newtheorem{lemma}{Lemma}%[theorem]

% \theoremstyle{definition}
% \newtheorem{defn}{Definition}%[section]
% \newtheorem{rem}{Remark}
% \newtheorem{ex}{Example}
% \newtheorem{problem}{Problem}%[section]

% \newcommand{\BibTeX}{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em\TeX}

% \newcommand{\N}{\mathbb{N}}  % natural numbers
% \newcommand{\R}{\mathbb{R}}  % real numbers
% \newcommand{\gm}{G}  % game
% \newcommand{\Gm}{\mathcal{G}}  % set of games
% \newcommand{\ps}{\mathcal{N}}  % player set
% \newcommand{\rs}{\mathcal{R}}  % resource set
% \newcommand{\ac}{\mathcal{A}}  % action set
% \newcommand{\wf}{\mathcal{W}}  % welfare function
% \newcommand{\poa}{\mathrm{PoA}}  % price of anarchy
% \newcommand{\ns}{\mathrm{NE}}  % nash
% \newcommand{\opt}{\mathrm{opt}}  % optimum
% \newcommand*{\Perm}[2]{{}^{#1}\!P_{#2}}  %permutation

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{document}

% %%% The following commands remove the headers in your paper. For final 
% %%% papers, these will be inserted during the pagination process.

% \pagestyle{fancy}
% \fancyhead{}

% %%% The next command prints the information defined in the preamble.

% \maketitle 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Introduction}

% Many significant engineering infrastructures are becoming increasingly distributed; this has led to a growing interest in the design and control of multi-agent systems. Developing this theory has a far outreach in its societal impact, not limited to sensor coverage in forest fire detection \cite{hefeeda2009forest}, wireless networks in smart grids \cite{liu2012wireless}, and even performance art \cite{carlson2020perceiving}. The fundamental gap between the design methodologies in multi-agent systems and traditional approaches in control and optimization arises from the strict informational and physical constraints of the individual agents. These constraints make it impractical to rely on a centralized decision-making process, and therefore require intelligent design of distributed protocols. As such, much of multi-agent literature focuses on the development and analysis of local decision making algorithms that give rise to desirable system-wide behavior. A standard approach to designing distributed algorithms is to pose an optimization problem with desired system properties stipulated by an objective function and physical and informational limitations of the agents captured as constraints in the problem \cite{nedic2014distributed}. Then, through careful consideration of the structure of the resulting optimization problem, a distributed algorithm is designed to give good approximate solutions. A critical question arises from this approach: \emph{How do we design good distributed algorithms when the underlying problem structure is not well known?} This question serves as the core motivation of this paper. Much of the previous literature assumes perfect knowledge of problem structure, however there are many problem instances where true system-level objective cannot be measured or estimated, either due to informational or computational limitations. For example, consider a sensor coverage scenario where a group of agents are responsible for covering and defending an area against malicious attacks. The precise location and value of certain assets are hidden from each agent due to security concerns, but a system designer generally like the agents to cover areas with higher valued assets. Even in this toy scenario, design of good distributed algorithms through the traditional approaches is not possible.
% %Not only should agents react independently and make decisions autonomously, they must also be able to coordinate with other agents.
% %A common approach to designing distributed decision rules is to work with the system level objective function and add coordination and physical limitations of the agents as constraints to the optimization problem. Then the structure of the problem is leveraged and the system level optimization is decomposed cleverly into a distributed optimization problem.

% Therefore in this paper, we turn to \emph{game theory} as an alternative approach to design and analyze multi-agent control algorithms in these imperfect information scenarios. Game theory provides a important set of tools deal with distributed design \cite{li2013designing}, \cite{marden2008distributed}. In particular, it allows for modular approach to distributed algorithms, where local utility functions are endowed on each agent and iterative algorithms lead to approximate solutions. A critical advantage of game theory is once the local utilities are designed, there is a set of readily available algorithms based on self-interested behavior that lead to relevant approximate solutions \cite{young1993evolution, marden2009payoff}. When the local utilities match the system objective, the design process resembles the traditional approach. However, due to the initially non-intuitive fact that assigning the system objective to local utilities is sub-optimal, design of efficient local utilities is a critical thrust of research. While there are suit of encouraging results on how to design local utilities \cite{paccagnan2018distributed, roughgarden2009intrinsic, gairing2009covering} for a variety of problem scenarios, design of efficient local utilities in situations with incomplete information and uncertain system environments is still relatively unexplored. Therefore, in this paper, we examine how surrendering the unrealistic assumption of agents having perfect system state information affects the resulting solutions stemming from different local utility designs.
% %However in this paper, we consider an alternate approach. We utilize a game-theoretic framework to decompose the design of distributive decision separately into local utility design an coordination algorithms. The problem of developing coordination algorithms has been already extensively looked at, so we consider the problem of utility design in this paper. We importantly note the non-intuitive result that setting local objectives to the system level objective is the best approach. This paper thus deals with utility design, where the local objectives are designed to promote emergent efficient system level behavior.

% \subsection{Related Works}

% The study of uncertainty in games is not new to the field of game theory - in fact one of the first significant contributions to game theory was due to John Harsanyi's seminal work in formulating \emph{incomplete information games}. Subsequently, there has been extensive research in these types of games, where every agent receives a noisy signal about the environment and make a decision accordingly. These differ from the standard game-theoretic notions, as agents beliefs about the true state as well as their beliefs on other agent's beliefs affect their decision \cite{mathevet2020information}. \cite{sagduyu2011jamming, billard1999learning, antoniades2003pursuit} all use incomplete information games to study multi-agent systems, either in wireless networks, team decision making, or pursuit and evasion. Incomplete information has also been used to model the bounded rationality of agents \cite{ortega2011information}. There has been previous work in local utility design in incomplete information games. \cite{roughgarden2015price}  provides a general method for the analysis and Analysis of resulting system efficiencies in certain incomplete information environments - \cite{garg2005price} extends the analysis to a class of congestion games. While this body of important work is relevant to our problem setting, we make two significant departures in assumptions from this literature: agents do not have a stochastic model of the system environment and no model on the information that other agents have. This is a significant assumption, for a relevant probabilistic model of the system environment may require significant sensing capabilities and/or significant computational capabilities. Thus our analysis will be quite different from this literature, and, in a loose sense, is comparable to the differences in stochastic and robust optimization.

% The literature in these "robust" environments is much less explored, but there is some work. \cite{weber1985method} considers how to generate a set of possible utility functions based on limited information.  \cite{akccay2012evolution} analyzes how biological interactions vary with informational asymmetries. \cite{aghassi2006robust} studies a distribution-free model of game theory through a new equilibium concept termed "robust-optimization equilibrium. \cite{meir2015playing} studies efficiency guarantees of local utilities, when all the players have the same wrong estimation of the system state. While related to our paper, we also study when it is also a mismatch of estimation of the system state between agents and design optimal design of local utilities. \cite{piliouras2016risk} is the closest paper, to the author's knowledge, that deal with such limited information scenarios. This paper deals with the how different sources of uncertainty and risk-averseness of agents can affect system performance. However, our paper also considers how to design local utilities that maximize system performance.

% %Perfectly rational decision-makers maximize expected utility, but crucially ignore the resource costs incurred when determining
% %optimal actions. However, computing such optimal actions is often very
% %difficult in practice due to prohibitive resource costs that are associated with the process of finding the optimal action. Bounded rationality \cite{ortega2011information}
% %Sensor networks (SN), and in general, unmanned systemnetworks (UMSN) are currently one of the strategic areas ofresearchindifferentdisciplines,suchascommunications,controls,and mechanics. These networks can potentially consist of alarge number of agents, such as unmanned aerial vehicles(UAV),unmanned ground vehicles(UGV),unmanned underwater vehicles (UUV), and satellites. Theadvantageofminimizingacostfunctionthatdescribesthe total performance of the team is that it can provide a bet-ter insight into performance of the entire team when comparedto individual agent performance indices. However, the potentialmain disadvantage of this formulation is clearly the requirementofavailabilityoffullinformationsetforcontroldesignpurpose.Inthe present work this problem is alleviated and the imposed in-formation structure of the team is taken into account by using alinearmatrixinequality(LMI)controlstrategybasedoncooperativegametheoryisappliedto the problem of cooperation in a team of unmanned systems.The main goal of the team is to reach at a common output,i.e. to have consensus \cite{ortega2011information}

% % There is one characteristic common to all of the above methods: each method
% % chosen to solve a given decision problem requires the decision maker to provide
% % preference judgments (information) until the method has determined, for example, one
% % utility function, or the complete ranking of alternatives, or the best alternative. These
% % methods do not usually address the problem of a decision maker's willingness or
% % ability to answer all of the necessary questions or to answer them with sufficient
% % precision. based on the incomplete information one is able to determine a set of utility functions
% % U(I) that is consistent with the incomplete information. This set of utility functions
% % can be used to reduce the set of decision-relevant alternatives as well as to give a first
% % incomplete prediction (based on ranges of part-worths) of the decision maker's
% % behavior  s. Based on the set U(I) the
% % additional assumptions lead to an exact solution that fits all information provided by
% % the decision maker. \cite{weber1985method}.
 
% % We prove an “extension theorem” for such games: price
% % of anarchy bounds for pure Nash equilibria for all induced full-information games extend automatically,
% % without quantitative degradation, to all mixed-strategy Bayes-Nash equilibria with respect to a product
% % prior distribution over players’ preferences. We also note that, for Bayes-Nash equilibria in games with
% % correlated player preferences, there is no general extension theorem for smooth games.
% % We give several applications of our definition and extension theorem. First, we show that many games of
% % incomplete information for which the price of anarchy has been studied are smooth in our sense. Our extension theorem unifies much of the known work on the price of anarchy in games of incomplete information.
% % Second, we use our extension theorem to prove new bounds on the price of anarchy of Bayes-Nash equilibria
% % in routing games with incomplete information.
% % where players are uncertain about each others’ payoffs.
% % Finally, a fundamental assumption behind ¨
% % the Nash equilibrium concept is that all players’ preferences are common knowledge,
% % and this assumption is violated in most auction and mechanism design contexts, where
% % participants have private information. \cite{roughgarden2015price}

% % Previous work in this area makes the complete information assumption,
% % that is, every agent knows deterministically the amount of traffic injected
% % by every other agent. Our work relaxes this by assuming that the amount
% % of traffic each agent wishes to send is known to the agent itself but not
% % to the rest of the agents; each agent has a belief about the traffic loads of
% % all other agents, expressed in terms of a probability distribution. In this
% % paper, we first set up a model for such network situations;
% % Our main results in this paper show that the bounds on price of anarchy for
% % incomplete information routing games are independent of the belief probability
% % distributions of the agents. This fact, in particular, implies that the same bounds
% % must hold for complete information routing games since they are the special case of
% % incomplete information games. \cite{garg2005price}

% % Our results point to a distinct avenue
% % for investigating how cooperation can evolve when the division
% % of benefits is flexible and individuals have private information
% %  Further, most research on biological cooperation focuses implicitly or explicitly on situations where individuals make
% % decisions under perfect information of their and others’ payoffs.
% % However, private information, where some individuals have access to information and others do not, is a feature of many biological and social interactions.
% % We suggest that these
% % failures occur because existing theory (14–16) assumes that reproductive skew evolves under perfect information about all relevant variables (17).We assume that these distributions
% % are attributes of the environmental variation, i.e., do not change
% % with the strategies of individuals or the game structure.
% % Our first kind of result is made possible by a celebrated theorem
% % from economics, the revelation principle (21), which allows us to
% % focus on a special class of simple games—direct mechanisms—that
% % can represent all possible equilibria in all possible games. \cite{akccay2012evolution}

% % We examine connections between the efficiency loss due to decentralization and the efficiency loss due to
% % uncertainty and establish tight performance guarantees for distributed systems in uncertain environments.
% % We present applications based on novel variants of atomic congestion games with uncertain costs, for which
% % we provide tight performance bounds under a wide range of risk attitudes. Our results establish that the
% % individual’s attitude toward uncertainty has a critical effect on system performance and therefore should be
% % a subject of close and systematic investigation.
% %  Such concerns about modeling imprecisions are especially relevant
% % when it comes to the study of socioeconomic phenomena since the “ground truth” of
% % human nature and decision making is inherently complex and intractable in its full
% % generality.
% % In contrast, the price-ofanarchy framework seems like an ideal testing ground for a quantitative study of
% % the implications of merging decision theory under uncertainty and game theory. In
% % this work, we wish to show how settings with uncertain payoffs coupled with riskaware agents may indeed not only be analytically tractable but also furthermore hold
% % the promise of revealing novel and sometimes surprising insights about well-studied
% % competitive settings.
% % The previous paragraph hopefully conveys that we can expect a wide range of attitudes toward uncertainty to materialize in our everyday experiences. Moreover, these
% % attitudes are not necessarily tied to the nature of the specific optimization problem.
% % They are typically
% % partitioned into the following two classes: (1) stochastic optimization, which utilizes the
% % ACM Transactions on Economics and Computation, Vol. 5, No. 1, Article 5, Publication date: October 2016.
% % Risk Sensitivity of Price of Anarchy under Uncertainty 5:7
% % distribution p over the uncertainty set and in some sense provides an “average-case”
% % analysis, and (b) robust optimization
% % As a result, the rank of each agent
% % on each machine (and therefore his or her respective experienced latency) is a random
% % variable. This defines a strategic game with uncertain cost functions. Our goal will be to
% % analyze the nature and efficiency of its stable states under different decision-theoretic
% % approaches to environmental uncertainty.
% % \cite{piliouras2016risk}


% % He assumed that the players
% % share a common-knowledge prior probability distribution over the type space. Harsanyi
% % suggested that each player would use this prior probability distribution, together with his
% % type, to derive a conditional probability distribution on the parameter values remaining
% % unknown to him.
% % Taking a different approach, other contributors to the game theory literature have
% % offered distribution-free equilibrium concepts for incomplete-information games. These
% % analyses address the possibility that distributional information is not available to the
% % players, or that they opt not to use potentially inaccurate distributional information. The
% % notion of an ex post equilibrium is the most common distribution-free solution concept
% % and is especially prevalent in the auction theory literature. 
% % ex post equilibria need not exist in
% % an incomplete-information game. \cite{aghassi2006robust}

% % In many situations a player may act so as to maximize a
% % perceived utility that is not exactly her utility function,
% % but rather some other, biased, utility.The implications of these limitations and biases on game
% % playing can be similarly described: in essence, the players
% % are playing the “wrong game,” by either applying some simple heuristics, or optimizing a dierent utility function fromNow, each player
% % i sees her utility as some other function ui, and thus we are
% % interested in the equilibria of the biased game G comprised
% % of modified utilities {ui}.Thus the PoA is not only robust to dierent notions of
% % equilibrium, but also to players that are not playing exactly
% % by the game specification.
% % Whether these modified utilities, and thus deviations from rational play, come
% % from a cognitive limitation, a behavioral bias, or a dierent
% % perception in regard to taxes or other payments, it is important to understand how the equilibria of the game are
% % aected. \cite{meir2015playing}.


% % Partial information induces a possible class of games, our paper takes the worst case instance out of the possible set of games. This is unlike Bayesian mechanism design where the probability distributions must be estimated or characterized.

% % Look at mechanism design papers with incomplete information?

% \subsection{Contributions}
% This paper generalizes previous work into distributed algorithm design, specifically local utility design, to the model a more realistic scenario where agents don't have perfect information or even a probabilistic model of the system. There has been few previous works that deal with this information setting, and to our knowledge, no other paper has addressed optimal design of local utilities. The main contributions of this paper includes:
% \begin{itemize}
%     \item In section \ref{sec:model}, we introduce the problem of utility design in uncertain environments, and introduce a relevant class of games in which to model uncertainties.
%     \item In section \ref{sec:comp}, a tractable linear program is formulated to give a tight characterization of efficiencies of the resulting solutions of the game with system uncertainties. Conversely, we also introduce a linear program to characterize an optimal utility design for these games.
%     \item In section \ref{sec:setcov}, we restrict our attention to the important class of set covering games with uncertainties. In this setting, we can get a direct characterization of efficiency under different forms of uncertainty and study how mismatches between estimated and realized system uncertainty can affect the optimality of local utilities.
% \end{itemize}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{The Model}
% \label{sec:model}

% In this paper, we consider the class of \emph{distributed resource allocation games} for a framework to study the relevant multi-agent problems. Since we would like to characterize the decision making process without directly attributing an explicit protocol, we utilize a game-theoretic description of the problem. Consider a game $\gm$ with an agent set $\ps = [1, n]$ and a set of finite resources $\rs = \{r_1, \dots, r_m\}$. Here, we use the denotation $[p, q]$ to represent the natural numbers between $p$ and $q$ inclusive, with $p < q$. Each agent $i \in \ps$ has an admissible action set $\ac_i \subseteq 2^\rs$ representing their capabilities. For a given allocation $a = (a_1, \dots, a_n) \in \ac = \ac_1 \times \dots \times \ac_n$, we define a welfare function $\wf: \ac \to \R $, describing the optimality of the resulting allocation by the agents, by
% \begin{equation}
%     \label{eq: welf}
%     \wf(a) = \sum_{r \in \rs}{W_r(a_r)},
% \end{equation}
% where $W_r: 2^{\ps} \to \R_{\geq 0}$ describes the added system welfare when a certain set of agents select the resource $r$ under the allocation $a$. This problem framework describes many relevant multi-agent scenarios. For completeness, we detail an example below.

% \begin{ex}[Vehicle-Target Assignment \cite{arslan2007autonomous}]
% Vehicle-target assignment problem models scenarios where the set of resources have an associated intrinsic value $v_r \in \R_{\geq 0}$, and there is a success probability for agent to cover the resource. This models a variety of situations, such as sensor coverage. For a success probability $0 \leq p \leq 1$,
% \begin{equation*}
%     \wf(a) = \sum_{r \in \rs}{v_r (1 - (1 - p)^{|a_r|})},
% \end{equation*}
% where $|a_r|$ denotes the number of agents that cover the resource $r$.
% \end{ex}

% The system objective is to find an optimal allocation $a^{opt}$ that maximizes the given welfare function in \eqref{eq: welf}. However, this problem is inherently intractable, and therefore requires generating approximate solutions. In this paper, we explore distributed approaches through intelligent design of agent's local objective functions. Here, we focus on a class of local objectives 
% \begin{equation*}
%     U_i(a_i, a_{-i}) = \sum_{r \in a_i} F_i(a_r),
% \end{equation*}
% where $F_i: 2^{\ps} \to \R_{\geq 0}$ represents the added utility for agent $i$ when a set of agents are covering the resource $r$ that $i$ also covers. We use the denotation $a_{-i}$ to refer to all the agents except agent $i$. In this paper, we would like to design $F_i$ such that the resulting efficiency of the game is optimal, without having a full characterization of $W_r$. In other words, we would like imbue local utilities for the agents under uncertainties of the system state.

% For this general game setup, there are few results on characterizing the inefficiency of the resulting solutions of the game. Therefore, we restrict our focus to \emph{local resource allocation games}. There are several positive results for efficiency characterization in this regime \cite{paccagnan2018distributed, chandan2019smoothness, vetta2002nash}, but unlike the previous literature, we consider incomplete information scenarios.

% Specifically, we examine the situation where $W_r(|a|_r)$ can be decomposed into $v_r \cdot w(|a|_r)$, where $v_r \geq 0$ represents the intrinsic value of the resource and $w: [1, n] \to \R_{\geq 0}$ describes the resource-agnostic added system welfare when $|a_r|$ agents cover resource $r$, i.e.
% \begin{equation}
%     \label{eq: welf}
%     \wf(a) = \sum_{r \in \rs}{v_r \cdot w(|a_r|)},
% \end{equation}

% In this paper, we would like to specifically explore scenarios where all the agents have different information about the world. Respective to local resource allocation games, we study scenarios where agents have imperfect information of all the value of the resources, i.e. $v_r$ is not known to any of the agents for any resource $r$. This might occur, for instance, due to noisy sensor measurements, and/or imperfect world knowledge. Specifically, for analysis, we assume that each agent's evaluation $v^i_r$ of the true value of the resource $v_r$ lies in a delta percentage interval, i.e. $v^i_r \in [(1-\delta) \cdot v_r, (1+\delta) \cdot v_r]$ for some specified $\delta \in [0, 1]$. Here $\delta$ characterizes the amount of information that the agents have about the world, as when $\delta = 0$, agents have perfect information, and when $\delta = 1$, the agents cannot differentiate if the resource is worth $v_r$ or $0$. Therefore, the actual realized utilities of the agents is 
% \begin{equation*}
%     U_i(a_i, a_{-i}) = \sum_{r \in a_i} v^i_r \cdot f(|a_r|).
% \end{equation*}
% where $f: \{1 \dots n\} \to \R$ represents the resource and agent agnostic distribution function describing the relative added utility to agent $i$ when $|a_r|$ number of agents cover resource $r$. 

% We denote the tuple $\gm := (\ps, \rs, \ac, \{v_r\}, \delta, w, f)$ as the game description of the defined local resource allocation problem, and $\Gm_{f, w, \delta}$ as the set of games with the welfare function $w$, the distribution function $f$, and the uncertainty parameter $\delta$. To determine the effectiveness of our utility design, we examine the resulting efficiency of the (pure) Nash equilibrium of the game, which we use throughout our paper as our solution concept. A \emph{Nash equilibrium} is an allocation $a^*$ that satisfies the following no-regret condition. 
% \begin{equation*}
%     U_i(a^*) \geq U_i(a_i, a_{-i}^*) \ \forall a_i \in \ac_i, \ \forall i \in \ps.
% \end{equation*}
% Characterizing the efficiency of the induced Nash equilibrium involves calculating the resulting \emph{price of anarchy},
% \begin{equation*}
%     \poa(\gm) := \frac{\min_{a \in NE(\gm)} \wf(a)}{\max_{a \in \ac} \wf(a)}
% \end{equation*}
% Price of anarchy has been used ... 
% Since we want to explore efficiency of our utility design over the class of games 
% $\Gm_{f, w, \delta}$, we extend the definition of price of anarchy,
% \begin{equation*}
%     \poa(f, w, \delta) := \inf_{\gm \in \Gm_{f, w, \delta}} \poa(\gm)
% \end{equation*}

% \begin{rem}
% Loss of coordination between agents has several immediate consequences, including the loss of the potential game structure. Potential games are well structured and guarantee the existence of pure Nash equilibrium. However, the next example shows that there can be a resource allocation game with misaligned information that does not have a pure Nash equilibrium. Therefore we restrict our considered class of games $\Gm_{f, w, \delta}$ to ones that do have Nash equilibrium. For other instances, notice that following arguments rely on generalized smoothness and therefore bound other equilibrium concepts as well, such as coarse correlated equilibrium, which are guaranteed to exist.
% \end{rem}

% \begin{ex}
% Consider the following resource allocation game with $2$ agents and $4$ resources $\{r_1, r_2, r_3, r_4\}$ each with a value $v_r = 1$. Let all agents have a distribution function $f = [1, 0]$, i.e. their utility is the value of all the resources they cover single-handedly without the the other agent. Also, let the agents valuations $\{v_r^i\}$ be $\{1+d, 1-d, 1+d, 1-d\}$ and $\{1-d, 1+d, 1-d, 1+d\}$ and their action sets $\ac_i$ be $\{\{r_1, r_2\}, \{r_3, r_4\}\}$ and $\{\{r_1, r_4\}, \{r_2, r_3\}\}$. It can be seen that this induces a best response cycle among the allocations, and therefore this game does not have a pure Nash equilibrium.
% \end{ex}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Computing price of anarchy}
% \label{sec:comp}

% In this section, we outline our main result, a tight characterization of the price of anarchy under a given welfare function, distribution function, and level of uncertainty.

% \begin{thm}
% \label{thm:LP}
% Consider a resource allocation game with $n$ number of agents, a welfare function $w \in \R^n_{> 0}$, a distribution function $f \in \R^n$ with $f(1) = 1$, and an uncertainty $\delta \in [0, 1]$, the price of anarchy of the game can be calculated by the following linear program
% \begin{align}
%     \label{eq:LP1}
%     \poa(f, w, \delta)^{-1} = \max_{\theta(a, x, b)} \sum_{a, x,  b}{w(b+x) \theta(a, x, b)} \\
%     \label{eq:LP2}
%     \mathrm{s.t.} \ \sum_{a, x, b}{\Big[\frac{1+\delta}{1 - \delta} a f(a+x) - b f(a+x+1)\Big] \theta(a, x, b) \geq 0} \\
%     \label{eq:LP3}
%     \sum_{a, x, b}{w(a+x) \theta(a, x, b)} = 1 \\
%     \label{eq:LP4}
%     \theta(a, x, b) \geq 0 \ \ \forall a, x, b
% \end{align}
% where $a, x, b \in \mathbb{N}$ such that $1 \leq a + x + b \leq n$.
% \end{thm}
\begin{proof}
First we show that $\poa(f, w, \delta)^{-1}$ is upper bounded by the optimal value of the proposed program. We can consider the reduced class of games $\Gm' \subset \Gm$ where all the agents have only $2$ actions, and without loss of generality, can assign one action to be the optimal action and the other to be a Nash equilibrium ($\ac_i = \{a_i^{\ns}, a_i^{\opt} \}$). Notice that the price of anarchy is not affected by only considering two actions. The overall structure of the linear program is
\begin{align}
    \label{eq:gform1}
    \poa(f, w, \delta)^{-1}  = V^*= \max_{\gm \in \Gm'_{f, w, \delta}} \wf(a^{\opt}) \\
    \label{eq:gform2}
    \mathrm{s.t.} \ U_i(a^{\ns}; \delta) \geq U_i(a_i^{\opt}, a_{-i}^{\ns}; \delta) \quad  \forall i \in \ps. \\
    \label{eq:gform3}
    \wf(a^{\ns}) = 1.
\end{align}
Notice that $\min \poa(\gm) = \max \poa^{-1}(\gm) = \max \frac{\wf(a^{\opt})}{\wf(a^{\ns})}$. Without loss of generality, we can scale down $v_r$ uniformly such that $\wf(a^{\ns}) = \sum_{r \in \rs}{v_r w(|a^\ns_r|)} = 1$, and, as such, derive the expressions in \eqref{eq:gform1} and \eqref{eq:gform3}.
We can partition the set of resources as
\begin{align*}
    \rs_{a^{\opt}_i} = \{r \in \rs : r \in a^{\opt}_i \setminus  a^{\ns}_i\} \\
    \rs_{a^{\ns}_i} = \{r \in \rs : r \in a^{\ns}_i \setminus a^{\opt}_i\} \\
    \rs_{a^{\opt}_i \cap a^{\ns}_i} = \{r \in \rs : r \in a^{\opt}_i \cap a^{\ns}_i\} \\
    \rs_{a^{\varnothing}_i} = \{r \in \rs : r \notin a^{\opt}_i \cup a^{\ns}_i\}.
\end{align*}

Now consider an arbitrary game $\gm \in  \Gm'_{f, w, \delta}$ with resources $\rs$, player valuations $\{v_r^i\}_{r \in \rs}$ for each player $i$ and true resource values $\{v_r\}_{r \in \rs}$. We can write the Nash constraint in \eqref{eq:gform2} for player $i$ with respect to resource allocation games as
\begin{equation*}
    \sum_{r \in a_i^{\ns}} v^i_r \cdot f(|a^{\ns}_r|) \geq \sum_{r \in a_i^{\opt}} v^i_r \cdot f(|(a_i^{\opt}, a_{-i}^{\ns})_r|).
\end{equation*}
Adopting the resource the partition, we can then rewrite the Nash condition as
\begin{align*}
    \sum_{r \in \rs_{a^{\ns}_i}} v^i_r \cdot f(|a^{\ns}_r|) + \sum_{r \in \rs_{a^{\opt}_i \cap a^{\ns}_i}} v^i_r \cdot f(|a^{\ns}_r|)  \\
    \geq \sum_{r \in \rs_{a^{\opt}_i}} v^i_r \cdot f(|(a_i^{\opt}, a_{-i}^{\ns})_r|) + \sum_{r \in \rs_{a^{\opt}_i \cap a^{\ns}_i}} v^i_r \cdot f(|(a_i^{\opt}, a_{-i}^{\ns})_r|).
\end{align*}
Canceling the terms in $\rs_{a^{\opt}_i \cap a^{\ns}_i}$, we get
\begin{equation*}
    \sum_{r \in \rs_{a^{\ns}_i}} v^i_r \cdot f(|a^{\ns}_r|) 
    \geq \sum_{r \in \rs_{a^{\opt}_i}} v^i_r \cdot f(|(a_i^{\opt}, a_{-i}^{\ns})_r|).
\end{equation*}
For any resource, $v^i_r \in [(1-\delta) v_r, (1+\delta) v_r]$, and so even if we enforce that $v^i_r = (1+\delta) v_r$ for all $r \in \rs_{a^{\ns}_i}$ and $v^i_r = (1+\delta) v_r$ for all $r \in \rs_{a^{\opt}_i}$ and $v^i_r = v_r$ for all other resources, the Nash condition is still preserved, and we compute the same price of anarchy as before. In other words, for any game $\gm \in \Gm'_{f, w, \delta}$, there exists another game $\gm'$ that has the price of anarchy, but where each player overvalues its allocation in Nash to the extreme and undervalues its allocation in $\opt$ to the extreme, and correctly identifies the value in the other allocations. Then we can restrict our attention to this scenario without loss of generality.

With this reduction, we can apply an approach inspired by \cite{paccagnan2018distributed}. We can define the parameters
\begin{align*}
    x_r &= |\{i \in \ps : r \in \rs_{a^{\opt}_i \cap a^{\ns}_i}\}|, \\
    a_r &= |\{i \in \ps : r \in \rs_{a^{\ns}_i}\}|, \\
    b_r &= |\{i \in \ps : r \in \rs_{a^{\opt}_i}\}|.
\end{align*}

Using the previously defined notation, we can define an alternate partition on the resources \begin{equation*}
    \rs(a, x, b) = \{r \in \rs : a_r = a, x_r = x, b_r = b \},
\end{equation*}
where $a, x, b \in \mathbb{N}$ such that $1 \leq a + x + b \leq n$. With this partition, its possible to write the welfare of the Nash allocation as 
\begin{align*}
    \wf(a^\ns) = \sum_{r \in \rs}{v_r w(|a^\ns_r|)} = \sum_{a, x, b} {\sum_{r \in \rs(a, x, b)}{v_r w(|a^\ns_r|)}} \\
    = \sum_{a, x, b} {\sum_{r \in \rs(a, x, b)}{v_r w(a_r + x_r)}} = \sum_{a, x, b} w(a + x) {\sum_{r \in \rs(a, x, b)}{v_r}}.
\end{align*}
Similarly, we can describe $\wf(a^\opt)$ as $\sum_{a, x, b} w(b + x) {\sum_{r \in \rs(a, x, b)}{v_r}}$. For the Nash constraint, we examine the relaxed condition $ \sum_i U_i(a^{\ns}; \delta) - U_i(a_i^{\opt}, a_{-i}^{\ns}; \delta) \geq 0$. Rewriting this condition with respect to the previously defined partition gives
\begin{align*}
    \sum_i U_i(a^{\ns}; \delta) - U_i(a_i^{\opt}, a_{-i}^{\ns}; \delta) = \\
    \sum_i \sum_{r \in \rs}{v^i_r (f(|a^{\ns}_r|) - f(|(a_i^{\opt}, a_{-i}^{\ns})_r|))} =\\
    \sum_{a, x, b} \sum_{r \in \rs(a, x, b)} \sum_i v^i_r (f(|a^{\ns}_r|) - f(|(a_i^{\opt}, a_{-i}^{\ns})_r|))  = \\
    \sum_{a, x, b} \sum_{r \in \rs(a, x, b)} \Big( [(1 + \delta) a f(a + x) v_r + x f(a + x) v_r] - \\ [ (1 - \delta) b f(a + x + 1) v_r + x f(a + x) v_r]\Big) = \\
    \sum_{a, x, b}  [(1 + \delta) a f(a + x) - (1 - \delta) b f(a + x + 1)] \sum_{r \in \rs(a, x, b)} v_r,
\end{align*}
where the fourth equality comes from the fact that agents overvalue the resource in the Nash allocation and undervalue the resource in the optimal allocation in our restricted class of games. Letting $\theta(a, x, b) = \sum_{r \in \rs(a, x, b)} v_r \geq 0$ and substituting the corresponding parametrizations, we have the linear program
\begin{align}
    \label{eq:LP1copy}
    W^* = \max_{\theta(a, x, b)} \sum_{a, x,  b}{w(b+x) \theta(a, x, b)} \\
    \label{eq:LP2copy}
    \mathrm{s.t.} \ \sum_{a, x, b}{\Big[\frac{1+\delta}{1 - \delta} a f(a+x) - b f(a+x+1)\Big] \theta(a, x, b) \geq 0} \\
    \label{eq:LP3copy}
    \sum_{a, x, b}{w(a+x) \theta(a, x, b)} = 1 \\
    \label{eq:LP4copy}
    \theta(a, x, b) \geq 0 \ \ \forall a, x, b.
\end{align}
Notice that for $W^*$ in \eqref{eq:LP1copy} and $V^*$ in \eqref{eq:gform1},  we have that $W^* \geq V^*$, since we have relaxed the Nash condition. Therefore $\poa(f, w, \delta)^{-1}$ is upper bounded by the optimal value. 

To show that $\poa(f, w, \delta)^{-1}$ is lower bounded by the optimal value, we outline a worst case game construction $\gm_{wc}$ inspired by the one in Theorem 2 in \cite{paccagnan2018distributed}. Let $\{\theta(a, x, b)\}_{a, x, b}$ be a feasible solution to the optimal program. For each possible $a, x, b$, and for each $i \in \ps$, we construct a resource $r$ with a value $\theta(a, x, b)/n$. The Nash and optimal actions for each player is assigned as follows 
\begin{align*}
    a_i^\ns = \cup_{j = 1}^n \{r(a, x, b, j) \mathrm{\ s.t. \ } a + x \geq 1 + ((j - i) \mod n)\} \\
    a_i^\opt = \cup_{j = 1}^n \{r(a, x, b, j) \mathrm{\ s.t. \ } b + x \geq 1 + ((j - i + b) \mod n)\}.
\end{align*}
The players valuations of each resource is $v^i_r = v_r (1 + \delta)$ if the resource is chosen in the Nash allocation, $v^i_r = v_r (1 -\delta)$ if the resource is chosen in the optimal allocation, and $v^i_r = v_r$ is the resource is not chosen in either or both allocations. It can be seen that this worst case game construction satisfies the constraints put forth in the proposed linear program. Since this worst case game has symmetric utilities, we have that $\frac{1}{n} \sum_i U_i(a^{\ns}; \delta) - U_i(a_i^{\opt}, a_{-i}^{\ns}; \delta) = U_i(a^{\ns}; \delta) - U_i(a_i^{\opt}, a_{-i}^{\ns}; \delta)$ for all players, and the price of anarchy bound is achieved by this worst case game. Therefore $\poa(f, w) \leq \poa(\gm_{wc}) = (W^*)^{-1}$ and our claim is shown.
\end{proof}

% Similar to the reasoning detailed in \cite{paccagnan2018distributed}, we can also define a linear program that computes the optimal design of a distribution function and the corresponding price of anarchy. We omit the details of the proof.

% \begin{cor}
% Consider a resource allocation game with $n$ number of agents, a welfare function $w \in \R^n_{> 0}$, and an uncertainty $\delta \in [0, 1]$. The $f_{\opt}$ that maximizes the price of anarchy is given as
% \begin{align*}
%     (f_{\opt}, \mu_{\opt}) \in \mathrm{arg} \min_{f \in \R^n,  \ \mu \in \R} \mu \\
%     \mathrm{s.t.} \ w(b + x) - \mu w(a + x) + \frac{1+\delta}{1 - \delta} a f(a + x) - b f(a + x + 1) \leq 0 \\
%     \mathrm{for \ all} \ a, x, b \in \mathbb{N} \ \mathrm{with} \  1 \leq a + x + b \leq n \\
%     f(1) = 1
% \end{align*}
% \end{cor}

% With this linear program defined, we can evaluate what the best design strategies are for different example scenarios.
% \\ EXAMPLES HERE.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Set Covering Applications}
% \label{sec:setcov}

% In this section, we restrict our analysis to set covering games, where the system welfare is the value of the resources covered, i.e. $w = \{1, \dots, 1 \}$. Set covering games are well studies and known to model a wide variety of practical applications. In this paper, we focus on the effect of delta uncertainty on the resulting efficiency of Nash equilibrium.

% For set covering games, we can characterize the efficiency of a proposed utility design with delta uncertainty through a closed form expression.

% \begin{prop}
% \label{prop:setpoa}
% For a given $f$ and $\delta$ and $n$ number of agents, the resulting price of anarchy is described as 
% \begin{align*}
%     \poa^{-1}(f, \delta) =
%     \max_{j \in \{1, \dots, n-1\}} \{\max \{\frac{1+\delta}{1-\delta} (j+1) f(j+1), \\
%     \frac{1+\delta}{1-\delta} j f(j+1) + 1,
%      \frac{1+\delta}{1-\delta} j f(j) - f(j+1) + 1 \} \}
% \end{align*}
% \end{prop}
% \begin{proof}
% First we construct the Lagrange dual of the program outlined Proposition \ref{thm:LP} as follows \begin{align*}
%         \min_{\lambda \geq 0,  \ \mu \in \R} \mu \\
%     \mathrm{s.t.} \ w(b + x) - \mu w(a + x) + \lambda [\frac{1+\delta}{1 - \delta} a f(a + x) - b f(a + x + 1)] \leq 0 \\
%     \mathrm{for \ all} \ a, x, b \in \mathbb{N} \ \mathrm{with} \  1 \leq a + x + b \leq n \\
% \end{align*}
% go through it?
% \end{proof}



% From this fact, we also have the following lemma
% \begin{prop}
% For a fixed number of agents $n$, the optimal distribution rule is as follows:
% \begin{equation}
%     \label{eq:setfopt}
%     \hat{f}_\delta(j) = \frac{\frac{1+\delta}{1-\delta}^{j-1} (j-1)! (\frac{1}{\frac{1+\delta}{1-\delta}^n (n-1)(n-1)!} + \sum_{k=j}^{n-1}{\frac{\frac{1+\delta}{1-\delta}^{-k}}{k!}})}{\frac{1}{\frac{1+\delta}{1-\delta}^n (n-1)(n-1)!} + \sum_{k=1}^{n-1}{\frac{\frac{1+\delta}{1-\delta}^{-k}}{k!}}},
% \end{equation}
% with a corresponding PoA of
% \begin{equation}
%     \label{eq:setpoaopt}
%     1 - \frac{1}{\frac{1}{\frac{1+\delta}{1-\delta}^n (n-1)(n-1)!} + \sum_{k=0}^{n-1}{\frac{\frac{1+\delta}{1-\delta}^{-k}}{k!}}}.
% \end{equation}
% \end{prop}
% \begin{proof}
% First we show that the price of anarchy is lower bounded by the proposed formula  with the corresponding proposed $f$. From the previous lemma, we have that 
% \begin{align*}
%         \poa^{-1}(f, \delta) \leq \mathcal{X} \mathrm{\ for \ any \ } \mathcal{X} \mathrm{\ s.t. \ } \\
%         \mathcal{X} \geq  \frac{1+\delta}{1-\delta} (n-1) f(n) + 1, \\
%         \mathcal{X} \geq \frac{1+\delta}{1-\delta} j f(j) - f(j+1) + 1 \quad j \in \{1, \dots, n-1\}
% \end{align*}
% where we removed the first set of constraints, and all but the last one of the second constraints. We can replace the set of inequalities with a system of equations as follows
% \begin{align}
%     \label{eq:optchar1}
%     \mathcal{X} = \frac{1+\delta}{1-\delta} (n-1) f(n) + 1 \\
%     \label{eq:optchar2}
%     \mathcal{X} = \frac{1+\delta}{1-\delta} j f(j) - f(j+1) + 1 \quad j \in \{1, \dots, n-1\}.
% \end{align}
% We can reformulate this system of equations as a recursive formula to generate a function candidate $f$ as follows
% \begin{align}
%     \label{eq:optrec1}
%     f(n) = 1 \\
%     \label{eq:optrec2}
%     f(j) = \frac{f(j+1) + \frac{1+\delta}{1-\delta}f(n)(n-1)}{\frac{1+\delta}{1-\delta} j}.
% \end{align}
% Iterating through this recursive equation and normalizing so that $f(1) = 1$ gives the proposed optimal distribution and that the price of anarchy is lower bounded by the proposed formula.

% For the upper bound, we construct a $n$ player worst case game inspired by \cite{gairing2009covering} as follows. All agents have $2$ actions: the Nash and optimal allocations.We divide the number of resources into $n+1$ levels, $\ell = \{0, \dots, n\}$, with the number of resources in each level being $(n-1)\frac{n-1)!}{(n - j)!}$ if $\ell > 0$ and $1$ resource in level $0$. The values of the resources in each level is $v_r = (\frac{1+\delta}{1-\delta})^\ell$. 

% To determine the Nash and optimal allocations of each agent, we first introduce a label for the resources in each level. The label for the resource in the $0^{th}$ level is $(1)$ and the labels for the resources in each level $\ell$ is the set of permutations $p \in \Perm{n}{\ell-1}$ minus the permutations with $1$ as the first index. The last index of the permutation $p$ denotes which agent selects the resource in the optimal allocation and $\{i \in \ps: i \notin p\}$ denotes which players select in the resource in the Nash allocation. However the exception is the resource in the $0^{th}$ level, where player $1$ selects that resource in both Nash and optimal allocations. For example, if the label for the resource $r$ is $(2, 3)$ for a $4$ player game, player $3$ selects that resource in the optimal allocation, and players $1$ and $4$ select that resource in the Nash allocation. Notice that for every resource in each level, $n - \ell$ players are selecting that resource in their respective Nash allocations.

% We first verify the Nash allocation is indeed a Nash action. We take note of the fact that at each level, there is a one-to-one correspondence between the resources with a label that has a last index of $i$ and a resource in the previous level that doesn't include the index $i$, from the truncation operation. Making the agent utilities explicit,
% \begin{align*}
%     U_i(a^\ns; \delta) = \sum_{\ell = 0}^{n} \sum_{r \in \rs^\ns_{i, \ell}} v_r^i f(n - \ell)
% \end{align*}
% where $\rs^\ns_{i, \ell}$ is the resources in level $\ell$ that are covered by agent $i$ under its Nash allocation. Now we have the following for all agents $i > 1$,
% \begin{align*}
%     U_i(a^\ns; \delta) &= \sum_{\ell = 0}^{n} \sum_{r \in \rs^\ns_{i, \ell}} (1 + \delta) v_r f(n - \ell) \\
%     &= \sum_{\ell = 0}^{n} |\rs^\ns_{i, \ell}| (1 + \delta) (\frac{1+\delta}{1-\delta})^\ell f(n - \ell) \\
%     &= \sum_{\ell = 0}^{n} |\rs^\opt_{i, \ell + 1}| (1 - \delta) (\frac{1+\delta}{1-\delta})^{\ell+1} f(n - (\ell + 1) + 1) \\
%     &= \sum_{\ell = 1}^{n} |\rs^\opt_{i, \ell}| (1 - \delta) v_r f(n - \ell + 1) \\
%     &= U_i(a_i^\opt, a_{-i}^\ns; \delta)
% \end{align*}
% where the first equality comes from the fact that the resources are extremely overvalued in the Nash allocation, the third equality comes from the one-one correspondence, the fourth equality comes from the fact that no resources in level $n$ are selected in Nash, and the fifth equality comes from the fact that the resources are extremely undervalued in the optimal allocation. 

% A similar approach holds for agent $1$ for levels $\ell \geq 1$, but for level $0$, we recall that the resource is selected in both the nash and optimal allocation. We importantly note that for this game construction, the utility is not affected by what distribution function we use. Additionally, for this game construction, under the Nash allocation, the first $0$ to $n-1$ levels are covered by the players, and under the optimal allocation, every resource is covered by a single player. We can explicitly write the welfare of this game for both allocations as
% \begin{align*}
%     W(a^{\ns}) = \sum_{r \in \rs}{v_r w(|a^\ns_r|)} = 1+ \sum_{\ell = 1}^{n-1} (n-1) \frac{\frac{1+\delta}{1-\delta}^\ell (n-1)!}{(n-\ell)!} \\
%     W(a^{\opt}) = \sum_{r \in \rs}{v_r w(|a^\opt_r|)} = 1 + \sum_{\ell = 1}^{n} (n-1) \frac{\frac{1+\delta}{1-\delta}^\ell (n-1)!}{(n-\ell)!}
% \end{align*}
% Therefore, we can verify an upper bound for price of anarchy as
% \begin{equation*}
%     \poa(f, \delta) \leq \poa(G_{f, \delta}) = \frac{W(a^{\ns})}{W(a^{\opt})} = 1 - \frac{1}{\frac{1}{\frac{1+\delta}{1-\delta}^n (n-1)(n-1)!} + \sum_{k=0}^{n-1}{\frac{\frac{1+\delta}{1-\delta}^{-k}}{k!}}}
% \end{equation*}
% and we show the claim.
% \end{proof}

% \begin{cor}
% The optimal PoA for any number of agents for a set covering game is $1-\frac{1}{e^{\frac{1-\delta}{1+\delta}}}$.
% \end{cor}
% \begin{proof}
% Note that $\poa(f, w)$ is monotonically decreasing with the number of agents $n$, as any game with $n_1$ agents can be recreated with $n_2$ agents when $n_2 \geq n_1$, where $n_2 - n_1$ agents have one trivial allocation, selecting a resource with value $0$. Therefore we examine the price of anarchy formula in equation \eqref{eq:setpoaopt} as $n \to \infty$. Then the limit is 
% \begin{align*}
%     \lim_{n \to \infty} 1 - \frac{1}{\frac{1}{\frac{1+\delta}{1-\delta}^n (n-1)(n-1)!} + \sum_{k=0}^{n-1}{\frac{\frac{1+\delta}{1-\delta}^{-k}}{k!}}} \\
%     = 1 - \frac{1}{\lim_{n \to \infty} \sum_{k=0}^{n-1}{\frac{\frac{1-\delta}{1+\delta}^{k}}{k!}}} = 1-\frac{1}{e^{\frac{1-\delta}{1+\delta}}}
% \end{align*}
% \end{proof}

% Its very likely that the system does not have perfect information on what the $\delta$ uncertainty is. Therefore we calculate the rice of anarchy of our designed $f$ at different $\delta$ interval.

% \begin{prop}
% Let $\hat{f}_{\delta}$ be the optimally designed $f$ for $\delta$ as in \eqref{eq:setfopt} and the realized mismatch ratio between agent evaluations and the true valuations be $\delta'$. If $n$ is high enough, the resulting price of anarchy $\poa(\hat{f}_{\delta}; \delta')$ for is
% \begin{equation*}
% \begin{array}{lr}
%         \frac{1+\delta'}{1-\delta'} - \hat{f}_{\delta}(2) + 1  & \mathrm{for \ } \delta \leq \delta',\\
%         (1 + \frac{1+\delta'}{1-\delta'} (n - 1) f(n))^{-1} & \mathrm{for \ } \delta \geq \delta'.
%         \end{array}
% \end{equation*}
% \end{prop}
% \begin{proof}
% We first note that as $\delta \to 1$, the recursive formula in \eqref{eq:optrec1} and \eqref{eq:optrec2} for the optimal distribution function is $f(n) = 1$ and $f(j) = \frac{n-1}{j}$. Normalizing to $f(1) = 1$ gives $f(j) = \frac{1}{j}$ for $j =  1, \dots, n-1$ and $f(n) = \frac{1}{n-1}$. Additionally, observe that as $\delta$ increases, the recursive formula in \eqref{eq:optrec2} produces a smaller $f(j)$ for a fixed $f(j)$, and so the normalized $f(j)$ increases as $\delta$ increases. Thus $f(j) \leq \frac{1}{j}$ for $j =  1, \dots, n-1$ for any $\delta$. We also take advantage of the fact that $f(j)$ is decreasing in $j$ and $f(1) = 1$ for any $\delta$.
% Now we look at the set of inequalities that characterize the price of anarchy in Proposition \ref{prop:setpoa}, the $\poa(f, \delta)^{-1} = \mathcal{X}$ with
% \begin{align}
%     \label{eq:setinequal1}
%     \mathcal{X} \geq \frac{1+\delta'}{1-\delta'} (j+1) f(j+1)  \quad j \in [1, n-1]\\
%     \label{eq:setinequal2}
%     \mathcal{X} \geq \frac{1+\delta'}{1-\delta'} j f(j+1) + 1  \quad j \in [1, n-1]\\
%     \label{eq:setinequal3}
%     \mathcal{X} \geq \frac{1+\delta'}{1-\delta'} j f(j) - f(j+1) + 1 \quad j \in [1, n-1]
% \end{align}
% We can eliminate the redundant inequalities to derive a closed form expression. For the first set of inequalities in \eqref{eq:setinequal1}, we have that 
% \begin{equation*}
%     \frac{1 + \delta'}{1 - \delta'} (j+1) f(j+1) \leq \frac{1 + \delta'}{1 - \delta'} \leq \frac{1 + \delta'}{1 - \delta'} - f(2) + 1 \ \ \  j \in [1,  n-2],
% \end{equation*}
% where the first inequality comes from $f(j+1) \leq \frac{1}{j+1}$ and the second inequality comes from $f(2) \leq f(1) = 1$. Inputting $j=1$ into the inequalities in \eqref{eq:setinequal3} gives the last term. For $j = n-1$, 
% \begin{align*}
%     \frac{1+\delta'}{1-\delta'} n f(n) = \frac{1+\delta'}{1-\delta'} (n-1) f(n) + \frac{1+\delta'}{1-\delta'} f(n) \\
%     \leq \frac{1+\delta'}{1-\delta'} (n-1) f(n) + 1,
% \end{align*} 
% where the second inequality comes from the fact that $f(n) \to 0$ as $n$ increases.
% For the second set of inequalities, we have that 
% \begin{align*}
%     \frac{1+\delta'}{1-\delta'} j f(j+1) + 1 &\leq \frac{1+\delta'}{1-\delta'}(j+1)f(j+1) - \frac{1+\delta'}{1-\delta'} f(j+1) + 1 \\
%     &\leq \frac{1+\delta'}{1-\delta'}(j+1)f(j+1) - f(j+2) + 1,
% \end{align*}
% where the second inequality comes from the fact that $\frac{1+\delta'}{1-\delta'}f(j+1) \geq 1 \cdot f(j+2)$ and matches the inequalities in \eqref{eq:setinequal3} for $j \in [1, n-2]$.

% We can also reduce the third set of inequalities with
% \begin{align}
%     \label{eq:prop331}
%     \frac{1+\delta'}{1-\delta'} j f(j) - f(j+1) + 1 = \\
%     \label{eq:prop332}
%     \frac{1+\delta'}{1-\delta'}(\frac{1-\delta}{1+\delta} f(j + 1) + f(n)(n-1)) - f(j+1) + 1 \leq \\
%     \label{eq:prop333}
%     (\frac{1+\delta'}{1-\delta'}\frac{1-\delta}{1+\delta} - 1) f(2) + (\frac{1+\delta'}{1-\delta'})f(n)(n-1)) + 1 
% \end{align}
% where the second equality comes substituting the recursive formula from \eqref{eq:optrec2} into $j f(j)$, and the inequality comes from rearranging terms and noting that $f(j+1)$ is decreasing in $j$ and achieves the maximum value at $j = 2$.
% Finally, the resulting set of inequalities is
% \begin{align}
%     \label{eq:setinequal12}
%     \mathcal{X} \geq \frac{1+\delta'}{1-\delta'} (n-1) f(n) + 1\\
%     \label{eq:setinequal22}
%     \mathcal{X} \geq \frac{1+\delta'}{1-\delta'} - f(2) + 1.
% \end{align}
% Lastly, we observe that when $\delta \leq \delta'$, $(\frac{1+\delta'}{1-\delta'}\frac{1-\delta}{1+\delta} - 1) \geq 0$ and the inequality in \eqref{eq:setinequal22} is tight and if $\delta \geq \delta'$, $(\frac{1+\delta'}{1-\delta'}\frac{1-\delta}{1+\delta} - 1) \leq 0$ and the inequality in \eqref{eq:setinequal12} is tight.
% \end{proof}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Conclusion}
% \label{sec:conc}
% In this paper, we've consider the problem of designing distributed algorithms for multi-agent scenarios under informational inconsistencies. This is necessary when the true system cannot be known or well-estimated, either due to computational or informational overhead. We study these incomplete information scenarios in the context of local resource allocation games, and use the price of anarchy to evaluate the quality of the emergent Nash equilibrium of the system. We first outline a tractable linear program to give a tight characterization of the price of anarchy under different levels of system uncertainties a well as a tractable linear program to outline the optimal utility design. Furthermore, we fully characterize the price of anarchy of the special subclass of set covering games with uncertainty and we examine the effect of uncertainty on optimality of the design utilities. This paper is an important first step to providing design strategies for multi-agents scenarios with more realistic assumptions on information availability to the agents.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % \section{Consensus}


% % Put consensus stuff here

% % \subsection{Different forms of uncertainty}
% % In this section, we develop a linear program to characterize the price of anarchy. First, we consider the situation where the agents' valuations of the resources can lie in different $\delta_i$ intervals. However, this program has a number of constraints that is combinatorial in the number of players. Therefore, to simplify the number of constraints, we then consider when all players have the delta uncertainty about the value of the resources. The resulting program aligns with one introduced in \cite{paccagnan2018distributed}, and has a resulting polynomial number of constraints.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % \section{Marden Proposal}

% % Multiagent Operations with Informational Inconsistencies 
 
% % In this section we consider a multiagent system operating in a vast environment seeking to accomplish a given system-level objective, e.g., surveillance or perimeter defense.  The operations of such systems require each individual agent to make local decisions in response to locally available information, which could pertain to information regarding the state of the mission or the behavior of the other agents in the system.  Given the vastness and complexity of these systems, it may the case that the information available to each agent is outdated or inconsistent with the true state of the system. Accordingly, the focus of this section is on understanding the impact of these informational inconsistencies on the resulting control design and performance guarantees.  
 
% % To ground the discussion above, consider a given multiagent system for surveillance in an environment with identified points of interest.  Suppose that each of the search agents has a characterization of this environment, and this characterization may differ from the true state of the system. How does a mismatch between the true state of the system and the agents’ perceived state of the system impact the efficiency of the emergent collective behavior?  What local coordination algorithms should be employed in such informationally inconsistent systems to optimize the quality of the emergent collective behavior? How should communication be employed to help remediate the issues caused by these informational inconsistencies?  Clearly, complete and comprehensive communication that enables all agents to know the true state of system is unrealistic. Accordingly, how should a communication network be employed to best assist the system?  For example, would it be more desirable for (i) there to be significant intra-agent communication which allows the agents to reach consensus on the state of the system (which may differ from the true state) or (ii) limited communication between a central operator a small collection of agents so that some agents know the true state of the system while other agents could views could differ substantially from both reality and one another?  

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \bibliographystyle{ACM-Reference-Format} 
% \bibliography{bibliography}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \end{document}
